Dynamic Walking of Bipedal Robots on Uneven Stepping Stones via Adaptive-frequency MPC

This paper presents a novel Adaptive-frequency MPC framework for bipedal locomotion over terrain with uneven stepping stones. In detail, we intend to achieve adaptive foot placement and gait period for bipedal periodic walking gait with this MPC, in order to traverse terrain with discontinuities without slowing down. We pair this adaptive-frequency MPC with a kino-dynamics trajectory optimization for optimal gait periods, center of mass (CoM) trajectory, and foot placements. We use whole-body control (WBC) along with adaptive-frequency MPC to track the optimal trajectories from the offline optimization. In numerical validations, our adaptive-frequency MPC framework with optimization has shown advantages over fixed-frequency MPC. The proposed framework can control the bipedal robot to traverse through uneven stepping stone terrains with perturbed stone heights, widths, and surface shapes while maintaining an average speed of 1.5 m/s.

==> Commands.tex <==
%!TEX root = ../Main.tex
% Defines commands to easily input variables and equations into the paper.

% Matrix commands for simple matrices
\newcommand{\pMat}[1]{\begin{pmatrix}#1\end{pmatrix}}
\newcommand{\bMat}[1]{\begin{bmatrix}#1\end{bmatrix}}
\newcommand{\BMat}[1]{\begin{Bmatrix}#1\end{Bmatrix}}
\newcommand{\aMat}[1]{\begin{Vmatrix}#1\end{Vmatrix}}
\newcommand{\mat}[1]{\begin{matrix}#1\end{matrix}}

% Pat commands
\newcommand{\cross}[1]{ {[#1]}_{\times} }

% Reference Frames
\newcommand{\IFrame}{\mathcal{I}}
\newcommand{\BFrame}{\mathcal{B}}
\newcommand{\COM}{CoM}

% State definitions
\newcommand{\roll}{\theta}
\newcommand{\pitch}{\phi}
\newcommand{\yaw}{\psi}

\newcommand{\rollhat}{\hat{\theta}}
\newcommand{\pitchhat}{\hat{\phi}}
\newcommand{\yawhat}{\hat{\psi}}



\newcommand{\dRoll}{\dot{\roll}}
\newcommand{\dPitch}{\dot{\pitch}}
\newcommand{\dYaw}{\dot{\yaw}}

\newcommand{\omegaX}{\omega_x}
\newcommand{\omegaY}{\omega_y}
\newcommand{\omegaZ}{\omega_z}

\newcommand{\dX}{\dot{x}}
\newcommand{\dY}{\dot{y}}
\newcommand{\dZ}{\dot{z}}

\newcommand{\quat}{\bm{q}}
\newcommand{\pos}{\bm{p}}
\newcommand{\angVel}{\bm{\omega}}
\newcommand{\vel}{\bm{v}}
\newcommand{\posDot}{\bm{\dot{\pos}}}
\newcommand{\posDotDot}{\bm{\ddot{p}}}
\newcommand{\quatDot}{\bm{\dot{\quat}}}
\newcommand{\angVelDot}{\bm{\dot{\angVel}}}

% Desired Variables
\newcommand{\xd}{\bm{x}_d}
\newcommand{\uref}{\bm{u}_{ref}}

% State component vectors
\newcommand{\quatV}{q_0 \\ q_x \\ q_y \\ q_z}
\newcommand{\quatVector}{\BMat{\quatV}}
\newcommand{\posV}{x \\ y \\ z}
\newcommand{\posVector}{\BMat{\posV}}
\newcommand{\angVelV}{\omegaX \\ \omegaY \\ \omegaZ}
\newcommand{\angVelVector}{\BMat{\angVelV}}
\newcommand{\velV}{\dX \\ \dY \\ \dZ}
\newcommand{\velVector}{\BMat{\velV}}

\newcommand{\rpyV}{\roll \\ \pitch \\ \yaw}
\newcommand{\rpyVector}{\BMat{\rpyV}}
\newcommand{\rpyDotV}{\dRoll \\ \dPitch \\ \dYaw}
\newcommand{\rpyDotVector}{\BMat{\rpyDotV}}

% Parameter Estimates
\newcommand{\state}{\bm{x}}
\newcommand{\stateDot}{\bm{\dot{\state}}}
\newcommand{\stateEstimate}{\bm{\hat{x}}}
\newcommand{\rFootEstimate}{\bm{\hat{r}}}
\newcommand{\forceEstimate}{\bm{\hat{F}}}
\newcommand{\rFootEstimatef}{\bm{\hat{r}}_f}
\newcommand{\forceEstimatef}{\bm{\hat{F}}_f}
\newcommand{\inputU}{\bm{u}}
\newcommand{\inputEstimate}{\bm{\hat{u}}}
\newcommand{\outputEstimate}{\bm{\hat{y}}}

% State and Input Vectors
\newcommand{\stateVector}{\BMat{\posV \\ \quatV \\ \velV \\ \angVelV}}
\newcommand{\stateVectorRed}{\BMat{\posV \\ \rpyV \\ \velV \\ \rpyDotV}}
\newcommand{\inputVector}{\BMat{\rFootEstimate_1 \\ \forceEstimate_1 \\ \rFootEstimate_2 \\ \forceEstimate_2 \\ \rFootEstimate_3 \\ \forceEstimate_3 \\ \rFootEstimate_4 \\ \forceEstimate_4}}

% Variable Transformations
\newcommand{\quatToRPY}{\bMat{\tan^{-1}\pMat{\dfrac{2\pMat{q_0q_1+q_2q_3}}{1-2\pMat{q_1^2+q_2^2}}}\\ \sin^{-1}\pMat{2\pMat{q_0q_2+q_3q_1}} \\ \tan^{-1}\pMat{\dfrac{2\pMat{q_0q_3+q_1q_2}}{1-2\pMat{q_2^2+q_3^2}}}}}
\newcommand{\omegaToRPYDot}{\bMat{\dfrac{\cos\pMat{\yaw}}{\cos\pMat{\pitch}} & \dfrac{\sin\pMat{\yaw}}{\cos\pMat{\pitch}} & 0 \\ -\sin\pMat{\yaw} & \cos\pMat{\yaw} & 0 \\ \dfrac{\cos\pMat{\yaw}\sin\pMat{\pitch}}{\cos\pMat{\pitch}} & \dfrac{\sin\pMat{\yaw}\sin\pMat{\pitch}}{\cos\pMat{\pitch}} & 1}}

% Time step definitions
\newcommand{\n}[1]{#1_n}
\renewcommand{\k}[1]{#1_k}
\newcommand{\nk}[1]{#1_{i}}

% Decision Variables Full
\newcommand{\inputVarsV}{\rFootEstimate \\ \forceEstimate}
\newcommand{\inputVarsVectorf}[1]{\BMat{\inputVarsV}_#1}
\newcommand{\decisionVarsVFull}{\inputVarsVectorf{1} \\ \vdots \\ \inputVarsVectorf{4} \\ \stateEstimate}
\newcommand{\decisionVarsVectorFull}[2]{\BMat{\decisionVarsVFull}_{#1,#2}}
\newcommand{\decisionArrayVFull}{\decisionVarsVectorFull{1}{1} & \hdots & \decisionVarsVectorFull{1}{K_1} & \hdots & \decisionVarsVectorFull{N}{1} & \hdots & \decisionVarsVectorFull{N}{K_N}}
\newcommand{\decisionArrayVectorFull}{\bMat{\decisionArrayVFull}}

% Decision Variables 
\newcommand{\decisionVarsV}{\stateEstimate \\ \inputEstimate}
\newcommand{\decisionVarsVector}{\BMat{\decisionVarsV}}
\newcommand{\decisionArrayV}{\decisionVarsVector_{1,1} & \hdots & \decisionVarsVector_{N,K_N}}
\newcommand{\decisionArrayVector}{\bMat{\decisionArrayV}}

% Simple Dynamics
\newcommand{\forces}{\bm{f}}
\newcommand{\torques}{\bm{\tau}}
\newcommand{\forceIEstimate}{\phantom{{}^\IFrame}\bm{\hat{f}}}
\newcommand{\torquesBEstimate}{^\BFrame\bm{\hat{\tau}}}
\newcommand{\RMatItoB}{^\BFrame\mathbf{R}_\IFrame}
\newcommand{\RMatItoBEstimate}{^\BFrame\mathbf{\hat{R}}_\IFrame}
\newcommand{\RMatBtoI}{^\IFrame\mathbf{R}_\BFrame}
\newcommand{\inputForceTorqueFunction}{ \hat{h}\!\pMat{\nk{\stateEstimate}, \nk{\inputEstimate}}}
\newcommand{\inputForceTorque}{\BMat{\phantom{{}^\BFrame}\forces \\ {}^\BFrame\torques}}
\newcommand{\inputForceTorqueMPC}{\BMat{\forceIEstimate \\ \torquesBEstimate}}
\newcommand{\forceTorqueTransform}{\bMat{\mathbf{I} & 0 \\ 0 & {\bm{R}_z^T(\yawhat)}}}
\newcommand{\uToForceTorqueMat}{\bMat{\mat{\mathbf{I} \\ \bMat{\bm{r}_1}_\times} & \hdots & \mat{\mathbf{I} \\ \bMat{\bm{r}_f}_\times}}}
\newcommand{\uToForceTorqueMatEstimate}{\bMat{\mat{\mathbf{I} \\ \bMat{\rFootEstimate_1}_\times} & \hdots & \mat{\mathbf{I} \\ \bMat{\rFootEstimate_f}_\times}}}
% Equation
\newcommand{\AMatnk}{{\bm{A}}_i}
\newcommand{\BMatnk}{{\bm{B}}_i}
\newcommand{\simpleDynamicsEq}{\AMatnk\nk{\stateEstimate}+\BMatnk\inputForceTorqueFunction+\bm{d}_i}
\newcommand{\simpleDynamics}{\stateEstimate_{i+1}=\simpleDynamicsEq}
% Matrix Linear
\newcommand{\AMatFull}{\bMat{\mathbf{I}_6 & \Delta t_i\mathbf{I}_6 \\ 0 & \mathbf{I}_6}}
\newcommand{\BMatFull}{\bMat{\frac{\Delta t_i^2}{2} \,{}^{\BFrame}\!\bm{I}^{-1} \\[.75ex] \Delta t_i\, {}^{\BFrame}\!\bm{I}^{-1} }}

\newcommand{\BMatFcull}{\bMat{\bMat{\frac{dt_n^2}{2}\mathbf{I}_6 \\ dt_n\mathbf{I}_6}\bMat{\frac{1}{m}\mathbf{I}_3 & 0 \\ 0 & ^\BFrame\bm{I}^{-1}}}}
	
	
	
% Full Dynamics
\newcommand{\sumForces}{\sum^\IFrame\bm{F}}
\newcommand{\sumTorques}{\sum^\IFrame\bm{\tau}}
\newcommand{\stateReducedVector}{\BMat{\pos \\ {}^\IFrame\!\bm{R}_{\BFrame} \\ \posDot \\ \angVel}}

\newcommand{\dynamicsReducedVector}{\BMat{
\posDot_c \\[.5ex]
{}^\IFrame\!\bm{R}_{\BFrame} \left[ {}^\BFrame \angVel\right]_\times \\[.5ex] 
\frac{1}{m}\forces - \bm{g} \\[.5ex]  
{}^\BFrame\,\overline{\!\bm{I}}{}^{-1}\pMat{{}^\BFrame\torques - {}^\BFrame \angVel\times {{}^\BFrame\,\overline{\!\bm{I}}}\,\,{\vphantom{\bm{I}}}^\BFrame\angVel}
}}


\newcommand{\stateDotReducedVector}{\BMat{\posDot_c \\ {}^\IFrame\!\dot{\bm{R}}_{\BFrame} \\ \posDotDot_c \\ {}^\BFrame\angVelDot}}

% Reference Input
\newcommand{\KPercent}{K_\%}
\newcommand{\pFootRef}{\bm{p}_{ref,f,xy,k} = \bm{\hat{p}}_{h,xy} + \posDot_{d,xy}T_{s}\pMat{\frac{1}{2}-\KPercent}+\\\pMat{\bm{\dot{\hat{p}}}_{xy} -\posDot_{d,xy}}\sqrt{\frac{\hat{p}_z}{\aMat{\bm{g}}}}\pMat{1 - \KPercent}}
			
% Error definitions
\newcommand{\stateError}{\bm{\tilde{x}}}
\newcommand{\inputError}{\bm{\tilde{u}}}
\newcommand{\stateErrorFull}{\xd-\outputEstimate}
\newcommand{\inputErrorFull}{\uref-\inputEstimate}
			
% Basic Cost Function
\newcommand{\basicArgs}{\stateEstimate, \hat{\bm{u}}}
\newcommand{\basicMin}{\underset{\basicArgs}{\text{min}}}
\newcommand{\basicCost}{J\pMat{\basicArgs}}
\newcommand{\basicCostFunction}{\basicMin\basicCost}
			
% MPC Function
\newcommand{\MPCSum}{\sum\limits_{n=1}^{N}\sum\limits_{k=1}^{\n{K}}}
%\newcommand{\MPCMin}{\underset{\stateEstimate, \inputEstimate}{\text{min}}}
\newcommand{\MPCMin}{\underset{\chi}{\text{min}}}
\newcommand{\stateCost}{\stateError^T\bm{Q}\stateError}
\newcommand{\inputCost}{\inputError^T\bm{R}\inputError}
\newcommand{\MPCCost}{\stateCost+\inputCost}
\newcommand{\MPCCostFunction}{\MPCMin\MPCSum\pMat{\MPCCost}_{n,k}}
			
% MPC Function Full
\newcommand{\MPCMinFull}{\underset{\stateEstimate, \inputEstimate}{\text{min}}}
\newcommand{\stateCostFull}{\pMat{\stateErrorFull}^T\bm{Q}\pMat{\stateErrorFull}}
\newcommand{\inputCostFull}{\pMat{\inputErrorFull}^T\bm{R}\pMat{\inputErrorFull}}
\newcommand{\MPCCostFull}{\stateCostFull+\inputCostFull}
\newcommand{\MPCCostFunctionFull}{\MPCMinFull\MPCSum\pMat{\MPCCostFull}_{n,k}}
			
% Constraints
\newcommand{\dynamicsConstraint}{\stateEstimate_{nk+1}=\simpleDynamicsEq}
\newcommand{\groundConstraint}{p_{z,f}=\hat{z}_g \pMat{p_{x,f}, p_{y,f}}}
\newcommand{\kinematicLegConstraint}{\aMat{\bm{r}_{h \to f}} \leq l_{f,max}}
\newcommand{\slipConstraint}{\bm{p}_{f,k+1} = \bm{p}_{f,k}}
\newcommand{\frictionConstraint}[1]{{-}\mu\bm{F}_{z,f}\leq\bm{F}_{#1,f}\leq\mu\bm{F}_{z,f}}
\newcommand{\frictionConeConstraint}{\frictionConstraint{x} \\ \frictionConstraint{y}}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% CONTACT
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\newcommand{\legState}{s}
\newcommand{\legStateScheduled}{\legState_{\phi}}
\newcommand{\legStateNotScheduled}{\bar{\legState}_{\phi}}
\newcommand{\legStateEstimated}{\hat{\legState}}
\newcommand{\contactState}{c}
\newcommand{\swingState}{\bar{\contactState}}
\newcommand{\contactStateScheduled}{\contactState_{\phi}}
\newcommand{\swingStateScheduled}{\bar{\contactState}_{\phi}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Support Polygon
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\phaseGain}{\Phi}
\newcommand{\adjLegP}{^{+}}
\newcommand{\adjLegM}{^{-}}

==> Sections/SystemOverview.tex <==
\section{System Overview}
\label{sec:sysoverview}


The optimization and control system block diagram is shown in Figure. \ref{fig:controlArchi}. 
We aim to achieve varied step lengths for each step in bipedal locomotion by adaptive-frequency MPC. The proposed framework is built around this controller. In order to allow more stable and efficient locomotion, we pair the MPC control framework with offline trajectory optimization to generate desired trajectories. Since MPC has a low sampling frequency and is determined by varied gait periods, we use a higher-frequency and task-oriented WBC scheme to allow more accurate trajectory tracking control. 


\begin{figure}[!h]
	\vspace{-0.3cm}
		\center
		\includegraphics[width=1 \columnwidth]{Figures/system2.pdf}
		\caption{{\bfseries System Block Diagram} Optimization and control architecture.}
		\label{fig:controlArchi}
		\vspace{-.2cm}
\end{figure}

The optimization framework uses terrain map to generate discrete optimization data including desired body CoM trajectory $\bm x_{des} \in \mathbb{R}^3$, desired foot position $\bm p_{n,des} \in \mathbb{R}^3$ for $n$th foot, and discrete sampling time $dt_i$ at time step $i$ for MPC. The CoM trajectory and foot positions are linearly-interpolated to have a sampling frequency at 1 $\unit{kHz}$ to match the frequency of swing leg control and WBC. The MPC accepts the optimization data at its native frequency due to the synchronization of sampling time. 
Reaction forces from MPC and swing leg control are input into WBC to be mapped to joint torques $\bm \tau  \in \mathbb{R}^{10}$.
The robot state feedback $\bm x \in \mathbb{R}^{12}$ include body Euler angles (roll, pitch, and yaw) ${\Theta = [\phi,\:\theta,\:\psi]}^\intercal$, position $\bm p_c$, velocity of body CoM  $\dot{\bm p}_c$, and angular velocity $\bm \omega$. Joint feedback $\mathbf q \in \mathbb{R}^{10}$ includes the joint positions of the bipedal robot. 
%The robot dynamics in simulation is solved by a continuous ODE solver and provides state feedback in continuous time. 
